IoT-based Big Data Analysis of School Buildings Performance

The utilization of IoT in the educational domain so far has trailed other more commercial application domains. In this chapter, we study a number of aspects that are based on big data produced by a large-scale infrastructure deployed inside a fleet of educational buildings in Europe. We discuss how this infrastructure essentially enables a set of different applications, complemented by a detailed discussion regarding both performance aspects of the implementation of this IoT platform, as well as results that provide insights to its actual application in real life, both from an educational and business standpoint.

==> chapter-apps.tex <==

\subsection{Usage Scenarios}

\gaia focuses on the following three energy scenarios, as also depicted in Figure~\ref{architecture.png}:

\myparagraph{Electricity:} \gaia monitors the electricity consumption at 
various time intervals (15 min, hourly, daily, monthly etc.). By using energy 
best practices, energy building modeling, user behavior modeling, energy data 
profiling techniques, and by real time observations in buildings (i.e., empty 
room or currently there is a lot of sunshine), provides recommendations to users 
so that they decrease the unnecessary operation of devices and, thus, 
reduce energy consumption.

\myparagraph{Heating:} \gaia monitors the energy consumption for heating purposes 
(gas, petrol) in longer periods of time (quarterly and annually). 
By using energy best practices, energy building 
modeling, user behavior modeling, energy data profiling techniques, and real 
time observations in buildings (i.e., good weather conditions), recommendations 
are provided to users in order to decrease the unnecessary operation 
of heating (or A/C) thereby reducing overall energy consumption.



\subsection{Other}




The platform also incorporates participatory sensing technologies for semi-automatic periodical collection of energy usage to acquire information in buildings where no IoT sensing elements are available, e.g., utilizing web/smartphone/social networking applications for acquiring information on room occupancy, usage of conditioning or special machinery, opening of windows, etc. The goal of \gaia is to include the users in the loop of monitoring the energy consumption in the buildings they use daily, thus making the first steps towards raising awareness, connecting the educational activities carried out at schools with their activities at their home environment and also engaging the parents and relatives at home. The teacher can initiate participatory sensing sessions during the courses so that students can use phones and tablets to gather data in real time and then review them in class (for more information see Sec.~\ref{sec:energy}).

The integrated sources of input are utilized to continuously provide direct feedback, custom-tailored to each particular learner/audience (i.e., kindergarten, school, university, parents). Direct feedback is provided via real-time displays (RTDs) installed at central locations in the buildings, published on school web sites, posted to social media, and also displayed on the users' smart phones and tablets. Direct feedback mechanisms are developed to address the immateriality of energy \cite{pierce2010materializing} and make it a visible entity by connecting it to the daily activities of students. Visual analytics are combined with recent advances in IoT sensing and pervasive computing technologies to provide an interactive environment that \textit{stimulates behavioural change on a frequent basis}. The energy consumption topic is included in the pedagogical activities of the schools incorporating educational aspects to promote energy literacy, convey information regarding historical data and comparative information with other buildings of similar characteristics (for more information see Sec.~\ref{sec:energy}). 

A series of social-networking applications are provided to set community-based incentives for pro-environmental behavioural change and promote collective consuming of resources. These applications utilize the already established relationship between users of the same school/department to provide \textit{community-based initiatives} to reduce their overall environmental footprint and increase environment friendly activities. A series of \textit{game-based competitions} further engage the students in learning how to improve the energy efficiency, and to encourage them to actually follow the learned practices. Research suggests that competitions can be effective in promoting environmentally responsible behavior \cite{gobel2010serious}. Historical data collected from the IoT infrastructure allows students to compete with each other on periodic intervals (e.g., per week/month/season) to further motivate eco-friendly behaviours. A combination of \textit{direct competition} among other groups of similar size, climate zone, socio-economic characteristics and past years (e.g., class 2016 vs recordings from class 2015) and \textit{indirect competition} against each group's own performance is followed. These competitions \textit{encourage spreading the word to larger groups}, allowing related persons, such as parents, friends, or neighbors, to participate and also \textit{appeal to positive emotions}, such as hope and enjoyment, as ways to changing individuals’ behaviors.

